A Survey on the Evolution of Stream Processing Systems

Stream processing has been an active research field for more than 20 years, but it is now witnessing its prime time due to recent successful efforts by the research community and numerous worldwide open-source communities. This survey provides a comprehensive overview of fundamental aspects of stream processing systems and their evolution in the functional areas of out-of-order data management, state management, fault tolerance, high availability, load management, elasticity, and reconfiguration. We review noteworthy past research findings, outline the similarities and differences between early ('00-'10) and modern ('11-'22) streaming systems, and discuss recent trends and open problems.

==> 4_State_management.tex <==
%!TEX root = main.tex

\section{State Management}\label{sec:state}

\subsection{A Brief History}
State is a concept that has been very central to stream processing. The notion of state itself has been addressed with many names such as ``summary'', ``synopsis'', ``sketch'' or ``stream table'' and it reflects the evolution of data stream management along the years. The early generation of the so called data stream management systems~\cite{babcock2002models} (circa 2000-2010) introduced the concept of \emph{continuous queries} on time-varying relations as an alternative to traditional DBMS queries which operated on predefined relations. Since the nature of evolving time-varying relations was potentially unbounded, the evaluation of continuous queries also hinted unbounded memory requirements to hold all the intermediate state needed to compute a precise answer. However, the lack of scalable state management solutions and managed out-of-memory state back then led to a series of ``best-effort'' or the processing systems~\cite{abadi2003aurora,arasu2004stream,chandrasekaran2003telegraphcq} for data streaming. These early systems made use of bounded in-memory data structures known as ``summaries'' which were predefined and limited to the query domain they supported (e.g., CQL~\cite{cql} operators in STREAM~\cite{arasu2004stream}).

A decade later, scalable data computing systems based on the MapReduce~\cite{dean2004mapreduce} architecture allowed for arbitrary user-defined logic to be scaled and executed reliably using distributed middleware and partitioned file systems. Following the same trend, many existing data management models were revisited and re-architectured with scalability in mind (e.g., NoSQL, NewSQL databases). Similarly, a growing number of scalable data stream processing systems~\cite{carbone2015apache,akidau2015dataflow,akidau2013millwheel,seep} married principles of scalable computing with stream semantics and models that were identified in the past (e.g. out-of-order processing~\cite{srivastava2004flexible,li2008out}). This pivoting helped stream management technology to lift all assumptions associated with limited state capacity and thus reach its nearly full potential of executing correctly continuous event-driven applications with arbitrary state. As of today, stream processors can compile and execute graphs of long-running operators with complete, user-defined state that is fault-tolerant and reconfigurable \cite{castro2013integrating,CarboneEF17,akidau2013millwheel}. Stream state management is an emerging research field that focuses on stateful operations and their guarantees within stream applications such as state access isolation~\cite{CarboneEF17} (e.g. read-committed), efficient state materialization~\cite{o1996log}, \cite{chang2008bigtable} and reconfiguration. 


\begin{figure*}[t!]
        \centering
        \includegraphics[width=.9\linewidth]{Figures/statefigs.pdf}
        \caption{Types of Data Stream State}
        \label{fig:streamstate}
\end{figure*}


\setlength{\tabcolsep}{5pt}
\begin{table*}[t!]
\smaller\centering
\caption{Types of State Supported by Stream Processing Systems.}
\label{tab:state}
\begin{tabular}{p{0.15\textwidth}|
                        p{0.07\textwidth}|
                        p{0.07\textwidth}|
                        p{0.07\textwidth}|
                        p{0.07\textwidth}|
                        p{0.07\textwidth}|
                        p{0.07\textwidth}|
                        p{0.07\textwidth}|
                        }
\hline
\textbf{System} &
\multicolumn{6}{c}{\textbf{Managed State}} &
\multicolumn{1}{c}{\textbf{External State}} \\

& In-memory
& Out-of-Core
& Partitioned
& Queryable
& Shared
& User-Defined
& 
\\
\hline
% Also passive
% The main problem is that the approach is not generally applicable
% since it depends on query semantics. Hence, \checkmark*
% Aurora*~\cite{cherniack2003scalable, abadi2003aurora}
% & %\multicolumn{1}{l}{\checkmark}
% &
% & 
% & %\multicolumn{1}{l}{slack}
% & %\multicolumn{1}{l}{\# tuples}
% &
% & 
 
% \\

% % Mentions in-flight data
% % Upstream: buffered 
% TelegraphCQ~\cite{shah2004highly}
% & 
% &
% & 
% &
% & 
% &

% & 
% \\

% % Heartbeat signifies liveness:
% %   Some techniques use punc- tuation [41], heartbeats [36], or statically defined slack
% %   [1] to tolerate bounded disorder and delays.
% Borealis~\cite{abadi2005design}
% & 
% &
% &
% & 
 
% &
% &
% & 
% \\

% Lossy failover is acceptable. Upon a server failure, processes are
% automatically moved to a standby server. The state of the processes,
% which is stored in local memory, is lost during the handoff.
% The state is regenerated using the input streams.
% Downstream systems must degrade gracefully.
% Nodes will not be added to or removed from a running cluster.
S4~\cite{neumeyer2010s4}
& \checkmark
& 
& \checkmark
& 
&

& \checkmark
& 
\\

Spark(1.0)~\cite{zaharia2012discretized}
& \checkmark
& 
& \checkmark
& 
& 
& 
& 
\\

% Cloud-based
% Provisioning
Seep~\cite{castro2013integrating}
& \checkmark
& \checkmark
& \checkmark
& 
& 

& \checkmark
& 
\\

% Stragglers
Naiad~\cite{murray2013naiad}
& \checkmark
& 
& \checkmark
& 
& 

& \checkmark
& 
\\

% Dynamic, on-demand reconfiguration: resilient substitution of vertices and sub-DAGs
% State and output dependency tracking
% Related work: S4, Storm, Trident, D-Streams
% Check out also Chronostream: Elastic stateful stream computation in the cloud
% which is based on Timestream
  % Large state maintenance
  % multi-tenant resource sharing
Timestream~\cite{QianHS13}
& \checkmark
& 
& \checkmark

&
& 
&
& 
\\

% * Millwheel/Dataflow (2015)
% 	-x-inmem (partially), x- out-of-core, partitioned, quer(external), x-shared(single read-write), x-shared, usd, external
Millwheel~\cite{akidau2013millwheel}
& \checkmark (partial)
& 
& \checkmark
& \checkmark

& 
& \checkmark
& \checkmark(BigTable)
\\

Storm~\cite{toshniwal2014storm}
& \checkmark
&
& \checkmark
& 
&
& \checkmark

& 
\\

% Synchronous checkpointing service. Under user control, the internal state
% of a running query can be persisted. The query can later be resumed by
% loading this state back, possibly on a different machine, and replaying
% data received since the checkpoint.
Trill~\cite{chandramouli2014trill}
& \checkmark
& 
& \checkmark
&
& 

& \checkmark
& 
\\

% % It can store state in an external database or it could keep the state in-memory,
% % but backed by HDFS (like how HBase works)
% Trident~\cite{CUSTOM:web/Trident}
% &
% & 
% &
% &
% & 

% &
% & 
% \\

% CetintemelDK14: Fault tolerance is achieved through a technique that combines
% command logging and periodic snapshotting.
% Leverage H-Store�s command logging mechanism to provide an upstream backup
% based fault tolerance technique for our streaming transaction workflows.
% 
% TatbulZM15: Exactly-once processing guarantee applies only to state that is internal to S-Store.
% To ensure the exactly-once processing guarantee, PE triggers are turned off
% during recovery; all transactions are replayed from the log,
% but no transactions will be repeated.
% Related work
% * ---
% StreamBase (2006) ?pdf?
% S-Store, (2014 VLDB demo, 2015 VLDB)
% 	- x-inmem,x-out-of-core, partitioned (h-store), quer(h-store), shared(h-store), x-usdt, external
% ---
S-Store~\cite{CetintemelDK14, TatbulZM15}
& 
& 
& \checkmark
& \checkmark 

& \checkmark
&
& \checkmark (h-store)
\\

Heron~\cite{KulkarniBF15}
& \checkmark
&
& \checkmark
&

&
& \checkmark
& 
\\

% * ChronoStream (2015 ICDE)
% 	-inmem, x-out-of-core, partitioned, x-quer, x-shared, usd, x-external
ChronoStream~\cite{wu2015Chronostream}
& \checkmark
& 
& \checkmark
&
& 
& \checkmark
& 
\\



% * Streamscope / StreamS (2016 NSDI)
% Provides fault-tolerance by detecting failures/stragglers and starting recovery
% Decouples upstream and downstream vertices with properties to facilitate
% failure recovery.
% cloud-based
% 	-inmem, x-out-of-core, partitioned, x-quer(external), x-shared(single read-write), x-shared, x-usd, x-external
Streamscope~\cite{LinHZ16}
& \checkmark
& 
& \checkmark
&
& 
& 
& 
\\

% Exactly-once output is achieved only when operators retract duplicate
% writes to external systems. This means exactly-once state.
System S~\cite{jacques2016consistent}
& \checkmark
& \checkmark
& \checkmark
&
& 
& \checkmark
& 
\\

% Very large state
% Container-based production environment
% Related work: Spark, Flink, S4, Storm, Heron, Borealis, Millwheel, Trident, Dataflow
% A changelog captures all updates done on the local store
% * Samza (2017 VLDB Industrial) - Samza: Stateful Scalable Stream Processing at LinkedIn
% 	- inmem, out-of-core(rocksdb), partitioned, ?-quer(external, partially at-least once), x-shared, usd
Samza~\cite{NoghabiPP17}
& \checkmark
& \checkmark
& \checkmark
&
& 
& \checkmark
& 
\\

% * Flink (State Management VLDB 2017)
% 	- inmem, out-of-core, partitioned, quer, x-shared, usd
Flink~\cite{carbone2015apache,CarboneEF17}
& \checkmark
& \checkmark
& \checkmark
& \checkmark (partial)
& 
& \checkmark
& 
\\

% Straggler mitigation by dividing work into small tasks
% The continuous processing mode recovers from node failures, but does
% not yet protect against stragglers or load imbalance.
% Catch up with input data
% Unprocessed output is tracked with WAL; in this sense output is checkpointed
Spark(2.3)~\cite{armbrust2018structured}
& \checkmark
& \checkmark
& \checkmark
& \checkmark (partial)
& 
& \checkmark 
& 
\\
\hline
\end{tabular}
\end{table*}




\subsection{Why do we need state?}
Unbounded computations are long running (years, even) and on every event, we need to change the state of an operator (e.g., a counter in Figure X). 

\subsection{Approximate vs. Exact State}
\asterios{here we will simply say that we will not deal with approximate state and sketches, after we define what approximate state is (vs. exact) referring to the seminal papers.}

\subsection{State Management Approaches}

Since state is an inseparable component to any event-based logic, every known stream processor, from early DSPSs, has allowed its use in some form, whether it was hidden or not from the user. In some cases (primarily first generations of systems) the underlying runtime was oblivious of any data structures and variables defined within the user scope. State management originates from the need to deal with transient failures, guaranteed processing and reconfiguration. Such requirements termed it necessary to design systems that are fully aware of state while being capable of managing transparently all operations affiliated with that state.

We observe two broad approaches when it comes to state management for stream processing i.e., families of system methodologies for persisting, updating and maintaining state throughout the course of a stream program. These two broad categories are 1) Internally Managed and 2) Externally Managed State, encapsulating whether state in a respective approach is materialized within or outside the scope of a ``computational task'', rather that being embedded within an OS process, thread, container or a physical local machine. In this section, we discuss all known variants of managed state that exist.
% , primarily in the cases of internally managed state as well as approaches that grant users with the ability to freely define, read and write state in stream programs.

\subsubsection{Locally Managed}

Locally-managed state is the most commonly adopted strategy for state management, since it enables direct, low-latency access to the physical state. Moreover, since the streaming system has the ability to manipulate state locally, it can allow for better garbage collection (e.g., when the contents of a window are no longer needed) but also for fine-tuned checkpointing algorithms (e.g., incremental checkpoints). Locally managed state can reside in memory or partially spilled to disk (e.g., on log-structure-merge data structures) as well as partitioned and accessed in numerous ways which we include in Table \ref{tab:state} and explain further below.

\paragraph{In-Memory:} One of the core design choices from early DSPSs to modern stream processors is the use of in-memory, transient state for fast access. In this case, the state is stored entirely in-memory, and most commonly within the same memory space as the streaming operator itself. Although access to the state has the lowest possible latency, the state size is bounded by the amount of available or pre-allocated memory. The simplest form of internal state is mutable data structures (Tree, or a Map). Naturally, in-memory state is supported by most existing approaches (managed or unmanaged).

\paragraph{Out-of-Core:} For reasons of memory limitations but also for fault-tolerance, a lot of systems make use of stable storage (HDD, SSD, etc.). The term most commonly used is ``out-of-core'' and it originates from the domain of out-of-core or ``external-memory'' algorithms designed to process data which is too large to fit into a machine's main memory at one time [TODO]. The intuition for stream processing is to use any allocated main memory together with auxiliary memory in order to store and access state. Different implementations of out-of-core state are provided nowadays as system plug-ins by production-grade stream processors which adopt a Log-Structure-Merge or Partial, In-memory B-tree [TODO] data structures to coordinate state operations between main and bulk memory units. Section~\ref{sec:FT} also mentions the benefits of these data structures to state snapshotting for fault tolerance and reconfiguration.

\paragraph{Partitioned:} Scale-out architectures of modern stream processors require some form of partitioning of streams. When a stream is partitioned by a given key, e.g., the clickstream on a per UserID basis, the state can also be naturally partitioned on a per UserID basis. For this reason, systems that are scalable and have internally-managed state management such as [TODO] also provide support for partiioned state. 

Partitioned state rings forward a set of challenges, during stream re-partitioning during which state has to migrate from one place to the other (we discuss state migration in \ref{fixme}). 
% Primarily in internally-managed state management approaches, it is necessary to model state in a way that allows re-partitioning when state needs to be shuffle to a different set of owning stream tasks.

\paragraph{Queryable:} For the most part, state is used internally to support operators such as windows (storing the contents of a window before it triggers), aggregates (e.g., storing counters) and joins (storing the Maps for implemetning a symmetric hash-join). However, external systems might need to query that state, for example, in order to query the current count of an aggregate or to query the current state of an automaton in a CEP topology. Moreover, querying state externally also enables programmers to debug their stream topologies. Queryable state, is a piece of state which one can query from the outside world. An altenrative to making state queryable is to publish each and every change of a given state (e.g., a counter or the contents of a window) for every event that changes that state \cite{secret} [SAYMORE]. Such an implementation, though, requires changing the semantics of the outputs of a stream; for instance, a window result comes with each new event arrival, which creates very verbose output channels). 

\paragraph{Shared:} 
\asterios{I think there is no real shared, internal state in any system today. Change my mind!}


\subsubsection{External State}
State can also be handed over to an external system, in order to simplify the design of a stream processor. For instance, users of Storm \cite{CUSTOM:web/Storm} typically store state in an external key-value store such as Cassandra \cite{lakshman2010cassandra}, while Millwheel \cite{akidau2013millwheel} stores its state on an external transactional system, namely Spanner \cite{corbett2013spanner} and BigTable \cite{chang2008bigtable}. There are good reasons for a system to hand-over its state to an external system. First, fault-tolerance is simplified as the external system takes care of persistence \footnote{Consistency of state is a serious concern in that case. We discuss this in \ref{fixme})}. Second, the system managing the state can re-partition or replicate that state without the need to coordinate with the streaming system. Third, external systems can query that state or subscribe to its changes. As seen in Table~\ref{tab:state}, the systems that make use of external state are Millwheel (through BigTable) and S-Store (through C-Store).


\subsubsection{User-Defined} Programmers in today's stream processing systems can often implement custom, user-defined logic in stateful operators. To this end, systems allow for defining custom state, which can be managed by the system itself. User-defined state unavoidably exposes some of the system's internals to its users. For instance, custom state in Apache Flink also requires the defition of functions to manage checkpoints and operator recovery as well as methods crucial for persistence (i.e.,serializers and deserializers). Such auxiliary operations on state can either be defined within the programming framework (e.g, State API in Apache Flink) or within external configuration files (e.g., in S4). In Table~\ref{tab:state} we see that the majority of existing systems support some form of user-defined state. 

\subsection{1st generation vs. 2nd generation}

\begin{itemize}
	\item bounded vs unbounded memory model
	\item synopses vs exact state
	\item query specific vs user-defined
	\item implicit vs explicit
	\item local vs distributed/partitioned
	\item on-heap vs out-of-core(LSM usage)
	\item transient stream input - logged input (logs)
	\item uncommitted vs read committed (snapshot isolation)
	\item application access - externally queryable
\end{itemize}

\subsection{Open Problems}
\begin{itemize}
	\item shared state
	\item state expiration
	\item complex data structures (e.g., graphs)
	\item nested operation state
\end{itemize}


==> 7_Related_Concepts.tex <==
%!TEX root = main.tex

\section{Related Concepts}

Reactive, dataflow programming, event-based, actors, time-series, temporal databases, active databases, complex-event processing.
Applications
Benchmarks

==> Makefile <==
pdf:
	@TEXINPUTS=.//: pdflatex -synctex=1 -interaction=nonstopmode --shell-escape main
all:
	@TEXINPUTS=.//: pdflatex -synctex=1 -interaction=nonstopmode --shell-escape main
	bibtex main
	pdflatex -synctex=1 -interaction=nonstopmode  --shell-escape main
	pdflatex -synctex=1 -interaction=nonstopmode  --shell-escape main
clean:
	find . -type f \( -name  '*.cut' -or -name  '*.xcp' -or -name  '*.thm' -or -name  '*.xml' -or -name '*.aux' -or -name  '*.auxlock' -or -name '*.figlist' -or -name '*eps-converted-to.pdf' -or -name '*.bbl' -or -name '*.fdb_latexmk' -or -name '*.synctex.gz' -or -name '*.blg' -or -name '*.log' -or -name '*.out' -or -name '*.toc' -or -name '*.lot' -or -name '*.lof' -or -name '*.loa' -or -name '*.fls' \) -exec rm -f '{}' \;



==> tutorial/1_Introduction.tex <==
%!TEX root = tutorial.tex

\section{Introduction}
During the last 10 years, applications of stream processing technology have gone through a resurgence, penetrating multiple and very diverse industries. Nowadays, virtually all Cloud vendors offer first-class support for deploying managed stream processing pipelines, while streaming systems are used in a variety of use-cases that go beyond the classic streaming analytics (windows, aggregates, joins, etc.). For instance, web companies are using stream processing for dynamic car-trip pricing, banks apply it for credit card fraud detection, while traditional industries apply streaming technology for real-time harvesting analytics. 

As seen in Figure~\ref{fig:overview}, during the last 20 years, streaming technology has evolved significantly, under the influence of database and distributed systems. The notion of streaming queries was first introduced in 1992 by the Tapestry system~\cite{terry1992continuous}, and was followed by lots of research on stream processing in the early 00s. Fundamental concepts and ideas originated in the database community and were implemented in prototypical systems such as TelegraphCQ~\cite{chandrasekaran2003telegraphcq}, Stanford's STREAM, NiagaraCQ~\cite{chen2000niagaracq}, Auroral/Borealis~\cite{abadi2003aurora}, and Gigascope~\cite{cranor2003gigascope}. Although these prototypes roughly agreed on the data model, they differed considerably on querying semantics \cite{cql,secret}. This research period also introduced various systems challenges such as sliding window aggregation \cite{arasu2004resource,li2005no}, fault-tolerance and high-availability \cite{shah2003flux,balazinska2008fault}, as well as load balancing and shedding \cite{tatbul2003load}. This first wave of research was highly influential to commercial stream processing systems that were developed in the following years (roughly during 2004 -- 2010), such as IBM System S, Esper, Oracle CQL/CEP and TIBCO. These systems focused -- for the most part -- on streaming window queries and Complex Event Processing (CEP). This era of systems was mainly characterized by scale-up architectures processing ordered event streams.

\begin{figure*}[t]
\centering
\includegraphics[width=.75\linewidth]{overview.pdf}
\vspace{-2mm}
\caption{\small An overview of the evolution of stream processing and respective domains of focus.}
\vspace{-1mm}
\label{fig:overview}
\end{figure*}

The last reincarnation of streaming systems has come as a result of stream processing research that started roughly after the introduction of MapReduce~\cite{dean2008mapreduce} and the popularization of Cloud Computing. The focus shifted towards distributed, data-parallel processing engines and shared-nothing architectures on commodity hardware. Lacking well-defined semantics and a proper query language, systems like Millwheel \cite{millwheel}, Storm, Spark Streaming~\cite{zaharia2012discretized}, and Apache Flink~\cite{carbone2015apache} first exposed primitives for expressing streaming computations as hard-coded dataflow graphs and transparently handled data-parallel execution on distributed clusters. With very high influence, the Google Dataflow model \cite{akidau2015dataflow} re-introduced older ideas such as out-of-order processing \cite{li2008out} and punctuations \cite{Tucker2003Exploiting} proposing a unified parallel processing model for streaming and batch computations. Stream processors of this era are converging towards fault-tolerant, scale-out processing of massive out-of-order streams.

At the moment of writing we are witnessing a trend towards using stream processors to build more general event-driven architectures \cite{kleppmann2019online}, large-scale continuous ETL and analytics, and even microservices \cite{operational-stream-processing}. These use-cases have led to application designs where the stream processor's \textit{state} has become a first-class citizen, visible to programmers \cite{CarboneEF17} but also to external systems.

%\vspace{-1mm}
%\subsection{Goal} 
We believe that this is the right moment to reflect on the similarities and differences between the two eras of streaming research and to assemble lessons learned. Moreover, we wish for this tutorial to bring forward important, but overlooked works that have played a vital role in today's streaming systems design. Finally, we aim to establish a common nomenclature for concepts which various open-source projects and commercial offerings are misusing.
\vspace{-3mm}


\subsection{Tutorial Outline} We will split this tutorial in three parts.

\stitle{1. Review of stream processing foundations}. This introductory part covers fundamentals of stream processing computation and system design. Specifically, we will cover languages and semantics, notions of time, out-of-order handling, and progress mechanisms.

\stitle{2. Evolution of system aspects}. The second part discusses the evolution of streaming system aspects. In particular, we will review state management practices, fault recovery, high availability and load management techniques.

\stitle{3. Emerging applications \& new requirements}. In the third part, we describe the characteristics and requirements of emerging streaming applications, focusing on real-time training and serving of ML models, event-driven applications, and microservice pipelines.
We then propose future research directions.


\subsection{Practical information}
\stitle{Scope.} This survey tutorial provides an overview of the two eras of research in stream processing, highlighting impactful work that has shaped modern streaming systems. We then discuss emerging applications, new requirements, and challenges to be addressed by the research community.

\stitle{Prior tutorials.}
The material proposed in this tutorial has not been presented before. Prior tutorials have either focused on a specific area (e.g., streaming optimizations \cite{schneider2013tutorial}) or on the broader area of event processing \cite{Etzion:2010:EPP:1920841.1921065}. To the best of our knowledge, the tutorial closest to ours was presented at DEBS 2014~\cite{heinze2014cloud} and covered Cloud Computing aspects of stream processing. Since then, modern streaming systems and applications have matured enough to allow for a deeper retrospective analysis and comparison.

\stitle{Duration \& target audience.}
The tutorial will last three (3) hours. 
Our target audience is graduate students, researchers, and practitioners from industry, who would benefit from a broader perspective of the evolution of stream processing. No prior knowledge of stream processing concepts is required as a prerequisite for attendance. 


==> tutorial/2_Foundations.tex <==
%!TEX root = tutorial.tex

\section{Review of Foundations}

The first part of our tutorial will be used to establish a common understanding of the basic notions of query languages, the effect of event ordering, as well as the time dimensions of streams. Finally, we will present various definitions of processing-progress in (dis)ordered streams.

\subsection{Languages and Semantics} Streaming query languages have been a subject of research since the very first days of stream processing. Virtually every attempt to create a standard language for streams has been an extension of SQL, by adding windowing and means to convert from streams to relations and vice versa. Most noteworthy examples were CQL~\cite{cql} and its derivatives~\cite{towards-standard-stream-sql, streamsql}. Later, dozens of works tried to extend the same standard for niche use-cases, with custom window types and aggregates; none of those attempts made it to standards.

Under the influence of MapReduce-like APIs, the majority of open-source streaming systems implemented functional/fluent APIs embedded in general purpose programming languages to hardcode Aurora-like dataflows. Till today, various communities are working on establishing a language for expressing computations which combine streams and relational tables, without a clear consensus.

\subsection{Time and Order}
Time and order lie at the heart of unbounded data processing.
Due to stochastic factors like network latency and operations
like shuffling and partitioning, data often arrives at a
streaming system out of order.
Besides the causes and effects of out-of-orderness, the tutorial will
examine the two fundamental strategies for processing out-of-order data.
The first  buffers data at the ingestion point
and allows batches of data to proceed in order~\cite{Tucker2003Exploiting,
srivastava2004flexible,millwheel,li2008out}.
The second, ingests out-of-order data as they arrive and
adjusts the computations in face of late data~\cite{Barga2006Consistent,
Mutschler2013Reliable}.

\subsection{Tracking Processing Progress}
Streaming systems need a way to track processing progress, i.e., how far along a stream has been processed. 
Progress tracking is required for triggers, windowing and state purging. 
Multiple measures have been devised to track progress. 
These measures are:
 punctuations~\cite{Tucker2003Exploiting},
 watermarks~\cite{akidau2015dataflow},
 heartbeats~\cite{srivastava2004flexible},
 slack~\cite{abadi2003aurora}, and
 frontiers~\cite{murray2013naiad}.
In the tutorial we will compare and contrast these mechanisms
with examples.


==> tutorial/3_Evolution.tex <==
%!TEX root = tutorial.tex

\newcommand{\NOTE}[1]{\textcolor{blue}{\textbf{NOTE}: #1}}
\section{Evolution of System Aspects}

Although the foundations of stream processing have remained largely unchanged over the years, important system aspects have transformed streaming systems into sophisticated and scalable engines, producing correct results in the presence of failures.


\subsection{State Management}
% It is not an understatement to say that state management changed stream processing.

State is a concept that has always been central to stream processing. The notion of state itself has been addressed with many names in the past, such as ``summary'', ``synopsis'', ``sketch'' or ``partitioned state'', and that reflects aspects of the evolution of data stream management over time. 
For example, several early systems adopted a bounded memory model for predefined stream operations such as window aggregates and joins with actual state being a best-effort, approximate summarization of necessary stream statistics for the operation at hand. In other cases, underlying stream runtimes had been oblivious of data structures and variables defined within the user scope of a stream application, leaving every challenge related to state management to the programmer. 

The need for explicit state management originates from the need to keep and automate the maintenance of persistent state for event-driven applications in a reliable manner. That includes the ability to store state beyond main memory, offer transactional processing guarantees, and allow for system reconfiguration~\cite{castro2013integrating,CarboneEF17,hoffmann19megaphone}. Such requirements made it necessary to design systems fully aware of stream state and capable of managing all associated operations transparently.

During our tutorial we are going to spend a considerable amount of time explaining the challenges related to partitioned state and processing guarantees, highlighting their impact to system design. We will further classify approaches into two broad directions: (i) internally-  \cite{castro2013integrating,CarboneEF17,NoghabiPP17} and  (ii) externally-managed state \cite{millwheel,meehan2015s,CetintemelDK14}, encapsulating whether state is managed within or outside a stream processor. We will discuss related aspects and technologies such as file systems, log-structured merge trees and related data structures, state expiration policies, window state maintenance, checkpoints, lineage-based approaches~\cite{zaharia2012discretized} and partitioning schemes for maintaining state.
\vspace{-3mm}
% In the early days of stream processing systems kept transient state that was lost on an operator's failure and lots of systems provided only a synopsis of the computations performed thus far since results were only approximate. The inability of stream processors to capture state in addition to the long history of approximate stream processing led to the misconception that stream processing can only be limited to non-mission critical, ``best-effort'' operations (e.g., Lambda Architecture~\cite{marz2015big}).

%The transition of stream processing systems to a distributed share-nothing architecture brought several interrelated problems to surface that go beyond fault tolerance~\cite{castro2013integrating} and include exposure to programming model, reconfiguration, state access isolation (e.g. read-committed), provenance and back-end materialization. Current approaches to stream state management can achieve a uniform and transparent solution to all of these issues via transactional processing methods such as consistent snapshotting~\cite{CarboneEF17}, batch discretization~\cite{zaharia2012discretized} or re-using existing DBMS transactional processing (e.g. S-Store~\cite{meehan2015s}, Millwheel/BigTable~\cite{millwheel}).

%combined with the adoption of distributed snapshots \cite{chandy1985distributed} in the stream processing domain, bringing globally consistent snapshots of a streaming system's partitioned state \cite{CarboneEF17, millwheel, SilvaZD16}.
%Consistent partitioned state. Today, stream processors can execute graphs of long-running operators with complete, user-defined state that is fault-tolerant and reconfigurable \cite{castro2013integrating,state2017carbone,millwheel} through sophisticated state management. Thus, streaming state management focuses on stateful operations and their guarantees within stream applications such as state access isolation \cite{state2017carbone} (e.g. read-committed), efficient state materialization \cite{o1996log, chang2008bigtable} and reconfiguration. State and its operations are all made explicit to the system \cite{fernandez2014making,castro2013integrating}. This unlocks the possibility of partitioning, persisting and committing changes in a consistent way, similar to DBMSs.




% \paris{At the dawn of the MapReduce era several attempts were made to enable general-purpose stream processing logic at scale. A popular example is Storm~\cite{CUSTOM:web/Storm}, an open-source system that allowed computation sharding. However, the system was agnostic of any form of state used (in-memory or external) and thus it was unable to scale, reconfigure or commit operations on state for fault recovery. } 


% \begin{itemize}
% 	\item transient vs persistent
% 	\item synopses vs exact state
% 	\item implicit vs explicit
% 	\item local vs distributed/partitioned
% 	\item on-heap vs out-of-core(LSM usage)
% 	\item transient stream input - logged input (logs)
% 	\item uncommitted vs read committed (snapshot isolation)
% 	\item application access - externally queryable
% \end{itemize}


\subsection{Fault Recovery and High Availability}
%Recovering from failures is fundamental when processing data continuously.
Fault recovery and high availability (HA) have been primary concerns for stream processing systems \cite{HwangBR05}. Apart from maintaining guarantees upon partial failures, stream processors also aim for low-latency executions. Therefore, recovery and HA mechanisms have to be non-obstructive to the stream execution at hand. 

We will review the evolution of two common HA techniques: \emph{active} and \emph{passive} standby. An \emph{active} standby runs two identical processing task instances in parallel and switches to the secondary instance when a fault occurs in the primary. This approach secures the highest level of availability and is the preferred option for critical applications. In contrast, a \emph{passive standby} instantiates a new instance of a failed operator on idle resources, such as a provisioned virtual machine~\cite{castro2013integrating, CarboneEF17}.
Passive standby has gained traction recently with the scale-out capacity of streaming systems. The modern version of passive standby entails transferring the computation code and the latest checkpointed state snapshot of a failed operator instance to an available compute node, such as a virtual machine or a container, and resuming operation from the latest checkpoint.

%To this end, we highlight the role of message brokers~\cite{kreps2011kafka}, which relay messages between an input source and a streaming system. They log input persistently, support multiple output partitions, and remember offset per output partition in order to replay messages from a specific offset.
%Replayable input allows streaming systems to recover from the latest checkpoint asking the broker to replay the messages from that point onwards.

%We will review the evolution of fault tolerance and high-availability strategies and look forward to the future as streaming systems increasingly become operational systems.

%\vasia{summary: ft is important in streaming because jobs run continuously and accumulate state.}
%\paris{Tackling partial failures transparently has always been one of the biggest challenges in data stream management. This is due to the fact that a stream processor, being a distributed system or not, may run for an arbitrarily long amount of time, possibly years, processing input events, accumulating state changes and producing output. Whereas, a network or process failure can at any point in time make all this work obsolete.}

%\vasia{summary: early systems applied FT in the context of quick process restart without providing system-wide guarantees. The lack of guarantees was partly due to the lack of re-playable inputs. Modern systems provide exactly-once semantics by leveraging distributed checkpoints and persistent re-playable inputs.}
%\paris{Fault recovery models~\cite{balazinska2009fault,balazinska2008fault} had primarily been proposed as a way for individual interconnected stream tasks to restart independently from failures using previously obtained snapshots to recover their execution state and reproduce computations that were possibly lost. Many of these proposed schemes also intermixed the concept of high availability~\cite{HwangBR05}, the ability to guarantee undisrupted processing despite potential failures. However, these approaches did not offer system-wide guarantees or access isolation levels similarly to how DBMSs did at the time. That was mainly due to loose assumptions regarding logged input and state as well as the lack of a clear specification of what application-wide processing guarantees can be for stream processing. Contemporary systems nowadays offer what is known as ``exactly-once processing'' guarantees~\cite{millwheel,state2017carbone,SilvaZD16,zaharia2012discretized}. We would like to bring forward some of the main impact factors that led to the development of strong processing semantics which are: 1) The usage of partitioned event logs (e.g., Kafka ~\cite{kreps2011kafka}) to offer logged and deterministic event queues for input, 2) The ability to make state explicit to the system \cite{castro2013integrating} as well as 3) The adaptation of snapshotting techniques~\cite{state2017carbone,millwheel,SilvaZD16,chandy1985distributed} to stream processing frameworks for transactional processing.}

\subsection{Elasticity and Load Management}
Due to the push-based nature of streaming inputs from external data sources, input rates might exceed system capacity causing performance degradation and increased latency. To counter this situation stream processing systems employ load management techniques. This is an area where the old and new systems contrast very vividly.

Early on, systems used \emph{load shedding} techniques to address excess traffic by dynamically dropping tuples. The load shedder system is expected to be capable of deciding when, where (in the query plan), how many, and which tuples to drop so that (i) latency improves to an acceptable level and (ii) results quality degrades only minimally.
In contrast, modern stream processing systems rely on managed partitioned state and the resource abundance of the Cloud and respond to workload variation via \emph{elasticity}~\cite{castro2013integrating, floratou2017dhalion, Kalavri2018three}. Elastic stream processors continuously monitor application performance and perform scale-out or scale-in actions of individual operators, ensuring correct migration of state partitions. In situations where input sources can control the data production rate, streaming systems can also utilize backpressure to inform the input sources to slow down.

==> tutorial/4_Applications.tex <==
%!TEX root = tutorial.tex


\section{Prospects}
Since its very beginning, stream processing has been conceived as a means of querying unbounded data sources in a relational fashion. The early systems and languages were designed as extensions of relational execution engines, with the addition of windows. As reflected by the current commercial stream processor offerings, traditional applications have been, for the most part, streaming analytical queries and CEP. Current streaming systems have evolved in the way they reason about completeness and ordering (e.g., out-of-order computation) and have witnessed architectural paradigm shifts that constituted the foundations of processing guarantees, reconfiguration, and state management. In this part of the tutorial, we summarize such observations from both application and system emerging needs. We then discuss how these new requirements can shape key characteristics of the future generation of data stream technology and outline open problems towards that direction.

\subsection{Emerging Applications} 

\stitle{Cloud Applications.}
At the moment of writing, we observe an interesting split in the design of modern Cloud programming frameworks. On one side of the spectrum, we witness stream processing APIs being implemented on top of Actor-like programming models -- examples of this is Orleans \cite{bykov2011orleans,bernstein2014orleans} and Akka Streams, as well as the streaming API of the Ray project \cite{moritz2018ray}. On the other side of the spectrum we see stream processing technology being used as a backend for Actor-like abstractions such as Stateful Functions\footnote{http://statefun.io}\cite{akhter2019stateful} tailored for Cloud deployment. These two paradigms (Actors on streams vs. streams on Actors) signify that the streaming and Actor programming paradigms and their associated system implementations might be converging, as a result of technology maturation and application requirements. We believe that stream processors can become full-fledged systems for backing Cloud services such as Virtual Actors~\cite{bernstein2014orleans} and Microservices \cite{operational-stream-processing, Goldstein2020providing}, capable of executing transactions, performing analytics, and embedding complex business logic of stateful services inside dataflow operators. 

%Modern event-based applications are challenging contemporary streaming system architectures, requiring not only higher scalability but also $i)$ better utilization with hardware (e.g., multicore) and modern  accelerators (e.g.,GPUs, FPGAs, RDMA) $ii)$ support for general-purpose event-based application building (vs. actor programming frameworks) $iii)$~transactional access to the internal state of operators (vs. external transactional databases).
%Throughout the tutorial we are going to present various new requirements and identify commonalities across the wider spectrum of data analytics and event-based applications, with real-life examples developed by users of open-source systems such as Apache Flink (e.g., ML pipelines, mission-critical air traffic management, dynamic pricing for car trips.). 
%We will further identify two broader system areas where these requirements are of high importance for further development of the capabilities of existing stream processing technology:

\stitle{Machine Learning.}
At the moment of writing, ML models are typically trained offline and a stream processor is used for model serving. Alternatively, the stream processor runtime is used for data distribution and coordination but complex operations, such as training and inference, are still mainly performed by specialized libraries. Thus, operators need to issue RPC calls to external ML frameworks and model servers adding both latency and complexity to the pipeline. Moreover, ML models need to be continuously updated, and oftentimes trained within the same pipeline as model serving. This means that the stream processor can cover the needs for online training, by offering constructs such as iterations, dynamic tasks, and shared state.

\stitle{Streaming Graphs.}
Another emerging application area is continuous analysis of graph streams, where events indicate edge and vertex additions, deletions, and modifications. Even though there exist many specialized systems for dynamic graph processing~\cite{Besta2020practice}, modern stream processors do not inherently support graph streaming use-cases. 
% Any analysis on complex data streams (hierarchical, nested, connected data) currently requires building ad-hoc solutions or performing snapshot-based computation. 
A prominent use-case is traffic and demand prediction for ride sharing services. Such an application needs to continuously compute shortest path queries with low latency and solve challenging online graph learning problems at the same time. It needs to simultaneously learn from, and analyze evolving graph inputs and other structured or unstructured types of static and dynamic data, such as driver and user locations, rush hours per area, neighborhood and points of interest (theaters, stadiums, etc.). The prediction tasks require generating graph embeddings using streaming random walks or online neural network training.
Another use-case is online network management in SDN controllers, where real-time events update the network topology and controllers execute continuous routing decisions, evaluate verification tasks, and find backup paths for each link in a streaming fashion.


\setlength{\tabcolsep}{4pt}
\begin{table}[t]
\small
\rowcolors{2}{gray!10}{gray!30}
\begin{tabular}{p{0.15\textwidth}
                p{0.015\textwidth}
                p{0.015\textwidth}
                p{0.015\textwidth}
                p{0.015\textwidth}
                p{0.015\textwidth}
                p{0.015\textwidth}
                p{0.015\textwidth}
                p{0.015\textwidth}
                p{0.015\textwidth}
                p{0.015\textwidth}
                }
 &
\begin{sideways}Programming Models\end{sideways} &
\begin{sideways}Transactions\end{sideways} &
\begin{sideways}Advanced State Backends\end{sideways} &
\begin{sideways}Loops \& Cycles\end{sideways} &
\begin{sideways}Elasticity \& Reconfiguration\end{sideways} &
\begin{sideways}Dynamic Topologies\end{sideways} &
\begin{sideways}Shared Mutable State\end{sideways} &
\begin{sideways}Queryable State\end{sideways} &
\begin{sideways}State Versioning\end{sideways} &
\begin{sideways}Hardware Acceleration\end{sideways}
\\
\hline
\textbf{Cloud Apps} &
\multicolumn{1}{c}{\checkmark} &
\multicolumn{1}{c}{\checkmark} &
\multicolumn{1}{c}{\checkmark} &
\multicolumn{1}{c}{\checkmark} &
\multicolumn{1}{c}{\checkmark} &
\multicolumn{1}{c}{\checkmark} &
&
\multicolumn{1}{c}{\checkmark} &
\multicolumn{1}{c}{\checkmark} &

\\
\textbf{Machine Learning} &
\multicolumn{1}{c}{\checkmark} &
&
\multicolumn{1}{c}{\checkmark} &
\multicolumn{1}{c}{\checkmark} &
&
\multicolumn{1}{c}{\checkmark} &
\multicolumn{1}{c}{\checkmark} &
\multicolumn{1}{c}{\checkmark} &
\multicolumn{1}{c}{\checkmark} &
\multicolumn{1}{c}{\checkmark}
\\
\textbf{Graph Processing} &
\multicolumn{1}{c}{\checkmark} &
&
\multicolumn{1}{c}{\checkmark} &
\multicolumn{1}{c}{\checkmark} &
&
&
\multicolumn{1}{c}{\checkmark} &
&
&

\\
\end{tabular}
\vspace{1mm}
\caption{Requirements for new applications}
\vspace{-3mm}
\end{table}


\subsection{The road ahead}
Several aspects of streaming systems could evolve further by exploiting next-generation hardware and incorporating ideas from programming languages, domain specific models, and distributed computing. During the tutorial we will discuss the following requirements that stem from new applications.
\vspace{2mm}

\stitle{Programming Models.}
Modern streaming systems allow developers to author streaming topologies with user-defined functions and functional APIs~\cite{carbone2015apache, armbrust2018structured} or some variant of streaming SQL~\cite{streamsql}.
However, these make the development of event-driven, Cloud applications very cumbersome. In fact, developers can only develop Cloud apps in a very low-level dataflow API. To build loosely-coupled Cloud apps, we need novel APIs that will allow developers to author simple high-level functions \cite{akhter2019stateful} or actor-like APIs \cite{moritz2018ray, bykov2011orleans} that can be compiled into streaming dataflows. 
Machine Learning and graph processing workloads require  programming models and abstractions that allow for iterations and complex data types (e.g., matrices, graphs), instead of tuple-like events. 

% Typically, cloud applications can be split in fine-grained components that can be developed and maintained autonomously.
% Their architecture enables their execution in container or serverless platforms with each component implementing a logical segment of the application logic.
% A programming abstraction for authoring each component should intuitively capture its input, output, state, and communication with other components as well as mask operational aspects like error and transaction management.
%We believe that a function-based {\sc api} is a natural fit for the above specification embodying a well-received programming abstraction.

\vspace{1mm}
\stitle{Transactions.}
Streaming systems lack transactional facilities to support advanced business logic and coordination as required by Cloud applications with the exception of S-Store \cite{meehan2015s}, which provides ACID guarantees on shared mutable state on a single machine.
Cloud applications feature many use-cases that span across components/services in a typically distributed environment.
Coordination of the components' processing is essential to safeguard state consistency and provide a single success or fail response that mirrors the successful recording of all state changes or none at all.
Applications require support by programming frameworks for
expressing transaction workflows that involve multiple components and for handling transaction abort cases and rollback actions in an automated manner.

\vspace{1mm}
\stitle{Advanced State Backends.}
A popular choice for a state backend in streaming systems is a key-value store~\cite{CarboneEF17, chandramouli2018faster}.
However, Cloud apps as well as machine learning and graph processing applications may require more sophisticated state such as dense matrices, large relational tables or an object-based blob storage.
Despite the chosen data model, persistently-backed state may need to be indexed and cached for fast access (think of product images qualified by a product id), support transactions including the possibility of a rollback (e.g., for online payments), or process complex analytical queries (e.g. on top of a Cloud data warehouse). Applications need a way to provide system-wide guarantees across the potentially disparate backends that comprise its overall state such as fault tolerance with strict consistency.

\vspace{1mm}
\stitle{Loops \& Cycles.}
%CA: Request/response, transaction lifecycle, cyclical communication between operators
Most dataflow systems today limit computation primarily in DAGs due to limitations in flow control (deadlock elimination) and monotonic event-time progress estimation. Nevertheless, there is a critical need for loops, either in the form of asynchronous event feedback or synchronously using bulk iterative semantics (Bulk and Stale Synchronous model variants). Asynchronous loops can enable request and response logic to support Cloud apps that demand two-way message exchange across functions (e.g., serverless) or actors or other more sophisticated mechanisms on dataflow tasks such as  concurrency control for transaction lifecycles. Synchronous loops are paramount for bulk iterative algorithms used in machine learning (e.g., Stochastic Gradient Descent) and are also critical for graph analytics that rely on iterative superstep synchronization to ensure consistent results. Therefore, the ability to express and execute different forms of loops will enable in the future a large set of computational models to be subsumed by stream processors. Despite existing efforts such as the Timely Dataflow model implemented in Naiad \cite{murray2013naiad}, there is still a need for intuitive and compositional integration of loops in existing systems at the programming model to allow users to express iterative operations while inter-playing seamlessly with event-time out-of-order processing \cite{li2008out}.

\vspace{1mm}
\stitle{Elasticity \& Reconfiguration.}
Streaming systems provide limited means for elasticity and reconfiguration actions, such as changing resource allocations and updating operator logic amidst a job execution.
Typically a stream processing job has to save its state, terminate its execution, and restart it with the refreshed operators.
For Cloud applications that have to be constantly online, this support is inadequate. Instead, applications need to apply code updates and hot fixes seamlessly to their operation without affecting the state or the processing of user requests.

%CA: code updates, resource utilization according to load

\vspace{1mm}
\stitle{Dynamic Topologies.}
%CA: new service components
The conventional means of expressing and executing dataflow streaming applications as statically compiled and scheduled graphs has been a limiting factor in both expressibility and performance for several types of computations. Many Cloud apps are dynamic by nature, requiring new instances of service components to be spawned on demand and execute their event-based logic independently from the ``main'' dataflow. Likewise, ML pipelines such as those seen in reinforcement learning are built around the notion of expanding computation dynamically during model exploration \cite{moritz2018ray}. The ability to compose dataflow topologies dynamically beyond static stream tasks can aid such application domains and also offer new performance capabilities to existing streaming use-cases such as work-stealing, parallel-recovery, skew mitigation and parallel execution of global aggregates (e.g., global windows) on demand.

\vspace{1mm}
\stitle{Shared Mutable State.}
A large set of applications from computational fields such as simulations, ML task-driven model training, and graph aggregations rely on the availability of shared mutable state, i.e., shared variables where multiple tasks can read and write. While this approach appears unconventional and challenging to integrate in purely-data parallel streaming systems, it carries great potential towards supporting non key-parallel modes of operation, model optimization algorithms and more complex data types.

\vspace{1mm}
\stitle{Queryable State.}
%CA: external queries to application state
Stream processing applications build and enrich persistent large state that represents dynamic relational tables, ML feature matrices or other types of derivative results from pre-processed and joined data from multiple input streams. While the standard interaction point with a stream processor has always been its input and output streams, internal state, currently a black box to the user, is becoming the main point of interest for many interactive and reactive data applications today. A step towards better reuse of computation is to allow dataflow applications to subscribe and gain read access to intermediate views of their respective states. This capability can further boost better interoperability across different Cloud apps and their internal components (e.g., stateful functions) as well as training and serving logic in ML. Related challenges in that direction include external query access isolation (e.g., snapshot) and flexible state management, which have only been partially considered in existing solutions (S-Store \cite{meehan2015s}, Flink point-queries \cite{CarboneEF17}).

\vspace{1mm}
\stitle{State Versioning.}
Streaming systems provide no explicit support for state versioning and state schema evolution. For Cloud and machine learning applications however, mutating the state schema is part of their lifecycle. Cloud applications change frequently, e.g., to introduce new services or update the current ones. As their state schema evolves, applications need a reliable way to version their state in order to continue operating consistently. Machine Learning applications also require state versioning. For instance, consider a continuous model serving pipeline (e.g., fraud detection) where a ML model needs to be updated while the pipeline is running. %The ability to update the state in a principled manner is yet to be seen in existing stream processors. 


\stitle{Hardware Acceleration.}
Hardware accelerators such as GPUs, TPUs, and FPGAs have become mainstream for certain ML workloads, especially when tensor computation is involved. While hardware acceleration has never really been a hard requirement for data streaming it starts to become more relevant, given the broadening capabilities of stream processors (e.g., Stream ML). Recent findings~\cite{koliousis2016saber,zhang2020hardware} have shown that stream-native operations (e.g., window aggregation) can also benefit from hardware accelerators such GPUs and Cloud FPGAs \cite{thomas2020fleet}. Overall, there is potential for more specialized code generation targeting diverse hardware architectures and general-purpose stream operators in the future \cite{zhang2020hardware}. Furthermore, apart from speedups, modern hardware can also lead to new capabilities in stream processing that were not previously considered possible. For example, new storage and network hardware can enable novel fault tolerance and state management mechanisms. Managed state currently resides mostly in \emph{volatile} memory and can be lost upon failure. The potential adoption of NVRAM and RDMA within compute clusters could shift current approaches from fail-stop to efficient fault-recovery models \cite{fernandez2014making,castro2013integrating}.


\begin{comment}

\noindent OLD TEXT
\begin{itemize}
    \item Flexible communication between operators, e.g. request-response, cycles, etc., and dynamic reconfiguration (support for general purpose event-based application building, Reliable Cloud applications)
    \item Programmer-friendly API for conveying business logic that closely resembles the way we write functions (support for general purpose event-based application building, Reliable Cloud applications)
    \item Transaction processing (support for general purpose event-based application building, Reliable Cloud applications)
    \item Execution hibernation for use in serverless environments (support for general purpose event-based application building, Reliable Cloud applications)
\end{itemize}

\vspace{-2mm}


\subsection{Trends}

Since its very beginning, stream processing has been conceived as a means of querying unbounded data sources in a relational fashion. The early systems and languages were designed as extensions of relational execution engines, with the addition of windows. As reflected by the current commercial stream processor offerings, traditional applications have been, for the most part, streaming analytical queries and CEP. Current streaming systems have evolved in the way they reason about completeness and ordering (e.g., out-of-order computation) and have witnessed architectural paradigm shifts that constituted the foundations of processing guarantees, reconfiguration, and state management. In this part of the tutorial, we summarize such observations from both application and system emerging needs. We then discuss how these new requirements can shape key characteristics of the future generation of data stream technology and outline open problems towards that direction.

Modern event-based applications are challenging contemporary streaming system architectures, requiring not only higher scalability but also $i)$ better utilization with hardware (e.g., multicore) and modern  accelerators (e.g.,GPUs, FPGAs, RDMA) $ii)$ support for general-purpose event-based application building (vs. actor programming frameworks) $iii)$~transactional access to the internal state of operators (vs. external transactional databases).
%$~real-time training and deployment of ML models on GPUs for fraud detection (vs. rules in CEP) $ii)$~ user-defined functions and custom business logic (vs. queries) and $iii)$~transactional access to the internal state of operators (vs. external transactional databases). 
Throughout the tutorial we are going to present various new requirements and identify commonalities across the wider spectrum of data analytics and event-based applications, with real-life examples developed by users of open-source systems such as Apache Flink (e.g., ML pipelines, mission-critical air traffic management, dynamic pricing for car trips.). We will further identify two broader system areas where these requirements are of high importance for further development of the capabilities of existing stream processing technology:

\noindent \textbf{I. Complex Analytics and DSLs:} Most streaming systems so far have implemented variations of stream querying capabilities, such as aggregates, joins and filters. At the moment, we notice a trend towards dynamic graph processing and machine learning which have only been modelled theoretically in the past with very small adoption rates from actual systems that are used in practice. For example, Ray~\cite{moritz2018ray} focuses on the fusion of data streaming, machine learning and actor programming. Similarly, a new generation of systems focuses on the intersection of batch and stream computational capabilities (Neptune~\cite{garefalakis2019neptune}, Arcon~\cite{meldrum2019arcon}). It is yet to be seen how domain specific variations of the streaming model can be implemented on top of existing or future stream processors. 




\subsection{Open Problems}
Several aspects of streaming systems could evolve further by exploiting next-generation hardware and incorporating ideas from programming languages, domain specific models, and distributed computing. During the tutorial we will discuss the following future research directions.

\noindent \textbf{Advanced state capabilities.} State expiration, deciding when and how to retire keys from streaming backends, is an open problem. Current solutions include defining a Time-To-Live parameter or some other fixed policy. Another important open challenge is 
the development of improved state-backing data structures~\cite{chandramouli2018faster} with better performance that this of LSM-trees, as well as support for complex state, such as graphs, that requires faster random access.

\noindent \textbf{Self-management and reconfiguration.} Streaming systems must be able to automatically adjust to dynamic environments, while guaranteeing quality of service and no data loss. However, the majority of stream processors place the burden of performance tuning and configuration to the user. A major challenge to providing automatic tuning is that any reconfiguration mechanism is required to safely migrate state, possibly across workers connected over a network, without causing performance degradation.

\noindent \textbf{Streaming query optimization.} 
Due to the long-running nature of queries, traditional cost-based optimization is not directly applicable to stream processing. Instead, a streaming optimizer needs to continuously monitor the environment and be capable of reacting quickly. The shared query execution plan approach and well-defined operator semantics of the first generation of streaming systems allowed them to employ several optimizations. On the contrary, due to their support for arbitrary UDFs, modern stream processors typically execute dataflow plans as provided by users.

\noindent \textbf{Support for new hardware.} Managed state currently resides mostly in \emph{volatile} memory and can be lost upon failure. The upcoming potential adoption of NVRAM and RDMA within large compute clusters could shift current approaches from fail-stop to efficient fault-recovery models \cite{fernandez2014making,castro2013integrating}. Hardware accelerators such as GPUs, TPUs, and FPGAs have also become mainstream for certain data analytical workloads, especially when tensor computation is involved. Recent studies (e.g., Saber~\cite{koliousis2016saber}) focus on accelerating stream operators with GPUs. There is potential for more specialized code generation targeting diverse hardware architectures and general-purpose stream operators in the future.

\end{comment}

==> tutorial/5_Future.tex <==
%!TEX root = tutorial.tex
